3D Photography using Context-aware Layered Depth Inpainting

We propose a method for converting a single RGB-D input image into a 3D photo - a multi-layer representation for novel view synthesis that contains hallucinated color and depth structures in regions occluded in the original view. We use a Layered Depth Image with explicit pixel connectivity as underlying representation, and present a learning-based inpainting model that synthesizes new local color-and-depth content into the occluded region in a spatial context-aware manner. The resulting 3D photos can be efficiently rendered with motion parallax using standard graphics engines. We validate the effectiveness of our method on a wide range of challenging everyday scenes and show fewer artifacts compared with the state of the arts.

==> figure/fig_ablation.tex <==
\newlength\qasb
\setlength\qasb{3.75cm}
\newlength\qasc
\setlength\qasc{1.95cm}
\newlength\qasep
\setlength\qasep{-7px}
\newlength\qasd
\setlength\qasd{1.45342465753\qasb}
%
\begin{figure*}[t]%
%
%
%
%
\parbox[t]{\qasb}{\vspace{0mm}\centering%
  \includegraphics[width=\qasb,trim=0 125 0 150,clip]%
	    {figure/ablation/woed}\vspace{-1mm}\\%
}%
\hspace{1mm}%
\parbox[t]{\qasc}{\vspace{0mm}\centering%
	\fbox{\includegraphics[width=\qasc,height=\qasc]%
	    {figure/ablation/woed_zoom_in_1}}\vspace{0.5mm}\\%
	\fbox{\includegraphics[width=\qasc,height=\qasc]%
	    {figure/ablation/woed_zoom_in_2}}%
}%
\hfill%
%
%
\parbox[t]{\qasb}{\vspace{0mm}\centering%
  \includegraphics[width=\qasb,trim=0 125 0 150,clip]%
	    {figure/ablation/diff}\vspace{-1mm}\\%
}%
\hspace{1mm}%
\parbox[t]{\qasc}{\vspace{0mm}\centering%
	\fbox{\includegraphics[width=\qasc,height=\qasc]%
	    {figure/ablation/diff_zoom_in_1}}\vspace{0.5mm}\\%
	\fbox{\includegraphics[width=\qasc,height=\qasc]%
	    {figure/ablation/diff_zoom_in_2}}\vspace{0.5mm}%
}%
\hfill%
%
%
\parbox[t]{\qasb}{\vspace{0mm}\centering%
  \includegraphics[width=\qasb,trim=0 125 0 150,clip]%
	    {figure/ablation/full}\vspace{-1mm}\\%
}%
\hspace{1mm}%
\parbox[t]{\qasc}{\vspace{0mm}\centering%
	\fbox{\includegraphics[width=\qasc,height=\qasc]%
	    {figure/ablation/full_zoom_in_1}}\vspace{0.5mm}\\%
	\fbox{\includegraphics[width=\qasc,height=\qasc]%
	    {figure/ablation/full_zoom_in_2}}\vspace{0.5mm}%
}%
%
%
%
%
\vspace{1.5mm}
%
%
\parbox[t]{\qasb}{\vspace{0mm}\centering%
    \hspace{0.920cm}%
		w/o edge inpainting
}%
\hspace{1mm}%
\parbox[t]{\qasc}{\vspace{0mm}\centering%
}%
\hfill%
\parbox[t]{\qasb}{\vspace{0mm}\centering%
    \hspace{0.910cm}%
		w/o color inpainting
}%
\hspace{1mm}%
\parbox[t]{\qasc}{\vspace{0mm}\centering%
}%
\hfill%
%
\parbox[t]{\qasb}{\vspace{0mm}\centering%
    \hspace{0.920cm}%
		Full model%
}%
\hspace{1mm}%
\parbox[t]{\qasc}{\vspace{0mm}\centering%
\hspace{0.5mm}
}%
%
%
%
\vspace{\figcapmargin}
\caption{Effect of different components in our proposed method. Without edge inpainting, the outcome quality is severely compromised. On the other hand, using color diffusion instead of inpainting model yields blurry artifacts around the foreground boundary. }

\label{fig:qualitative_ablation}
\end{figure*}


==> figure/fig_artifact.tex <==
\newlength\qlsa
\setlength\qlsa{4.10cm}
\newlength\qlsb
\setlength\qlsb{1.6cm}

% inverse aspect ratios of our results
\def\qlaa{0.3153988868274583}
\def\qlab{0.2565217391304348}
\def\qlac{0.3196969696969697}

\begin{figure}[h!]%
\centering%
\parbox[t]{\qlsa}{\vspace{0mm}\centering%
  \includegraphics[width=\linewidth, height=\qlsb]{figure/rebuttal/artifact_ours}\vspace{0.3mm}\\%
  \includegraphics[width=\linewidth, height=\qlsb]{figure/rebuttal/benefit_ours}\vspace{-1mm}\\%
	Our results}%
\hfill%
\parbox[t]{\qlsa}{\vspace{0mm}\centering%
  \includegraphics[width=\linewidth, height=\qlsb]{figure/rebuttal/artifact_baselines}\vspace{0.3mm}\\%
  \includegraphics[width=\linewidth, height=\qlsb]{figure/rebuttal/benefit_baselines}\vspace{-1mm}\\%
	$[$55$]$}%
%\caption{Qualitative results compare to ~\cite{zhou2018stereo}.}
\label{fig:artifact}
\end{figure}

==> figure/fig_cascaded_depth_edge.tex <==
\begin{figure}[t]
% \mfigure{0.22}{figs/teaser/ex2a_img.jpg} \hfill
% \mfigure{0.22}{figs/teaser/ex2b_img.jpg} \hfill
% \mfigure{0.22}{figs/teaser/ex2c_img.jpg} \hfill
% \mfigure{0.22}{figs/teaser/ex2d_img.jpg}

\vspace{\figcapmargin}

\caption{
\tb{TITLE.} 
\jiabin{Show two examples in two rows
1st column:  Context-hole with depth discontinuity
2-4 columns: gradually extended depth edges for each iteration.
}
}
\label{fig:cascaed_depth_edge}
\end{figure}

==> figure/fig_complex.tex <==
\begin{figure}[h]
\includegraphics[width=0.4\linewidth]{figure/rebuttal/fig_7_revised}
\label{fig:revised_fig7}
\end{figure}

==> figure/fig_motivation.tex <==
\begin{figure}[t]
% \jbox{\textwidth}{0.3\linewidth}
\begin{tabular}{cc}
\mfigure{0.45}{figure/motivation/motive_1.pdf} &
\mfigure{0.45}{figure/motivation/motive_2.pdf} 
\end{tabular}
\caption{\textbf{The need for localized inpainting.} A region can either be the \red{hole} and \blue{context} for inpainting at the same time. 
(\emph{Left}) The layer (b) should be used as the \blue{context} to fill the \red{hole} occluded by layer (a).
(emph{Right}) The layer (c) should be used as the \blue{context} to fill the \red{hole} occluded by layer (b). Synthesizing the regions occluded by layer (a) and (b) with adaptive context regions simplifies the task.
}
\label{fig:motivation}
\end{figure}

==> figure/fig_qualitative_ablation.tex <==
\begin{figure}
\centering
% Pairs that seem to have easily noticeable differences
\setlength{\tabcolsep}{0.01em}
\begin{tabular}{cccc}
\mfigure{0.25}{figure/linked_edges/input} &
\mfigure{0.25}{figure/linked_edges/input} &
\mfigure{0.25}{figure/linked_edges/input} &
\mfigure{0.25}{figure/linked_edges/input}  \\
Input & No color. & No discont. & Full Model\\

\mfigure{0.25}{figure/linked_edges/raw_disparity} &
\mfigure{0.25}{figure/linked_edges/input} &
\mfigure{0.25}{figure/linked_edges/input} &
\mfigure{0.25}{figure/linked_edges/input} \\
Depth &(Zoom in patch). & (Zoom in patch). & Full Model\\

\end{tabular}
\caption{\textbf{Effect of different components in our proposed method.} \blue{Temporary placeholder.}}
\label{fig:qualitative_ablation}

\end{figure}

==> figure/fig_revise_fig7.tex <==
\begin{figure}[h]
\includegraphics[width=\linewidth]{figure/rebuttal/fig_7_revised_ver2}
\label{fig:revised_fig7}
\end{figure}

==> figure/fig_simple_diffusion.tex <==
\newlength\qlsa
\setlength\qlsa{4.10cm}
\newlength\qlsb
\setlength\qlsb{1.0mm}
\newlength\flca
\setlength\flca{2.7cm}
\def\qlaa{1.0}
\def\qlab{1.0}
\def\qlac{0.3196969696969697}
\parbox[t]{\qlsb}{\vspace{0mm}\centering%
    \includegraphics[width=\qlsa,height=\qlaa\qlsa]%
        {figure/rebuttal/diffuse_depth}\vspace{\qlsb}\\%
    }%
\hfill%
\parbox[t]{\qlsb}{\vspace{0mm}\centering%
    \includegraphics[width=\qlsa,height=\qlaa\qlsa]%
        {figure/rebuttal/dl_depth}\vspace{\qlsb}\\%
    }\vspace{1mm}\\%
\begin{figure}[t]
\fbox{\includegraphics[width=\flca,trim=0 350 0 200,clip]{figure/rebuttal/dl_depth}}%
\hfill%
\fbox{\includegraphics[width=\flca,trim=0 350 0 200,clip]{figure/rebuttal/diffuse_depth}}%
%
%
%
\caption{
    Simple diffusion.
}
\label{fig:diffusion}
\end{figure}

==> overview.tex <==
\section{Overview}
\label{sec:overview}

% Introduce your problem with a toy example

% This figure illustrate the overall process of the algorithm, starting from inputs, processing steps, and outputs. Use forward references the figures with the corresponding equations and sections in the paper.
\input{figure/fig_overview}
